A Term-based Approach for Generating Finite Automata from Interaction Diagrams

Non-deterministic Finite Automata (NFA) represent regular languages concisely, increasing their appeal for applications such as word recognition. This paper proposes a new approach to generate NFA from an interaction language such as UML Sequence Diagrams or Message Sequence Charts. Via an operational semantics, we generate a NFA from a set of interactions reachable using the associated execution relation. In addition, by applying simplifications on reachable interactions to merge them, it is possible to obtain reduced NFA without relying on costly NFA reduction techniques. Experimental results regarding NFA generation and their application in trace analysis are also presented.

==> images/coreg/graph.tex <==
\begin{tikzpicture}
\node[draw] (q0) at (0,0) {\includegraphics[scale=.3]{images/coreg/n1.png}};
\node[draw, circle, fill=black,left=.2cm of q0] (i0) {};
\draw[->] (i0.east) -- (q0.west |- i0.east);
%
\node[draw,right=1cm of q0] (q1) {\includegraphics[scale=.3]{images/coreg/n2.png}};
\draw[->] (q0) -- node[midway,above] {\small$\hlf{l_1}!\hms{m_1}$} (q1);
%
\node[draw,right=1cm of q1, double, double distance=2pt] (q2) {\includegraphics[scale=.3]{images/coreg/n4.png}};
\draw[->] (q1) -- node[midway,above] {\small$\hlf{l_2}?\hms{m_1}$} (q2);
%
\node[draw,below=.75cm of q0] (q3) {\includegraphics[scale=.3]{images/coreg/n3.png}};
\draw (q0) edge[bend right=30,->] node[midway,left] {\small$\hlf{l_3}!\hms{m}$} (q3);
\draw (q3) edge[bend right=30,->] node[midway,left] {\small$\hlf{l_2}?\hms{m}$} (q0);
%
\node[draw,below=.75cm of q1] (q4) {\includegraphics[scale=.3]{images/coreg/n5.png}};
\draw (q1) edge[bend right=30,->] node[midway,left] {\small$\hlf{l_3}!\hms{m}$} (q4);
\draw (q4) edge[bend right=30,->] node[midway,left] {\small$\hlf{l_2}?\hms{m}$} (q1);
%
\node[draw,right=1cm of q4] (q5) {\includegraphics[scale=.3]{images/coreg/n8.png}};
\draw (q2) edge[bend right=30,->] node[midway,left] {\small$\hlf{l_3}!\hms{m}$} (q5);
\draw (q5) edge[bend right=30,->] node[midway,left] {\small$\hlf{l_2}?\hms{m}$} (q2);
%
\draw[->] (q3) -- node[midway,above] {\small$\hlf{l_1}!\hms{m_1}$} (q4);
\draw[->] (q4) -- node[midway,above] {\small$\hlf{l_2}?\hms{m_1}$} (q5);
\end{tikzpicture}


==> images/diff/coreg_seq/1/graph.tex <==
\begin{tikzpicture}
\node[draw] (i1) at (0,0) {\includegraphics[scale=.3]{images/diff/coreg_seq/1/n1.png}};
\node[draw,right=1cm of i1] (i2) {\includegraphics[scale=.3]{images/diff/coreg_seq/1/n3.png}};
%
\draw[->] (i1) -- node[midway,above] {\small$\hlf{l_1}!\hms{m_2}$} (i2);
\end{tikzpicture}

==> images/diff/coreg_seq/2/graph.tex <==
\begin{tikzpicture}
\node[draw] (i1) at (0,0) {\includegraphics[scale=.3]{images/diff/coreg_seq/2/n1.png}};
\node[draw,right=1cm of i1] (i2) {\includegraphics[scale=.3]{images/diff/coreg_seq/2/n3.png}};
%
\draw[->] (i1) -- node[midway,above] {\small$\hlf{l_1}!\hms{m_2}$} (i2);
\end{tikzpicture}

==> images/nfa/nosimpl/term2.tex <==
\begin{tikzpicture}[every node/.style = {shape=rectangle, align=center}]
\node (o) {$strict$} [level distance=0.75cm,sibling distance=1.25cm]
    child { node (o1) {$\varnothing$} }
    child { node (o2) {$i$} };
\end{tikzpicture}

==> images/nfa/nosimpl/term3.tex <==
\begin{tikzpicture}[every node/.style = {shape=rectangle, align=center}]
\node (o) {$strict$} [level distance=0.75cm,sibling distance=1.25cm]
    child { node (o1) {$seq$} [sibling distance=1cm]
      child { node (o11) {$strict$}
        child { node (o111) {$\varnothing$} }
        child { node (o112) {$\hlf{l_1}?\hms{m_1}$} }
      }
      child { node (o12) {$\hlf{l_1}!\hms{m_2}$} }
    }
    child { node (o2) {$i$} };
\end{tikzpicture}

==> images/nfa/nosimpl/term4.tex <==
\begin{tikzpicture}[every node/.style = {shape=rectangle, align=center}]
\node (o) {$strict$} [level distance=0.75cm,sibling distance=1.25cm]
    child { node (o1) {$seq$} [sibling distance=1cm]
      child { node (o11) {$\varnothing$} }
      child { node (o12) {$\hlf{l_1}!\hms{m_2}$} }
    }
    child { node (o2) {$i$} };
\end{tikzpicture}

==> images/nfa/nosimpl/term5.tex <==
\begin{tikzpicture}[every node/.style = {shape=rectangle, align=center}]
\node (o) {$strict$} [level distance=0.75cm,sibling distance=1.25cm]
    child { node (o1) {$seq$} [sibling distance=1cm]
      child { node (o11) {$\varnothing$} }
      child { node (o12) {$\varnothing$} }
    }
    child { node (o2) {$i$} };
\end{tikzpicture}

==> images/nfa/term1.tex <==
\begin{tikzpicture}[every node/.style = {shape=rectangle, align=center}]
\node (o) {$loop_S$} [level distance=0.75cm,sibling distance=1.25cm]
    child { node (o1) {$alt$} []
      child { node (o11) {$seq$}
        child { node (o111) {$strict$} [sibling distance=1.1cm]
          child { node (o1111) {$\hlf{l_2}!\hms{m_1}$} }
          child { node (o1112) {$\hlf{l_1}?\hms{m_1}$} }
        }
        child { node (o112) {$\hlf{l_1}!\hms{m_2}$} }
      }
      child { node (o12) {$\hlf{l_2}?\hms{m_3}$} }
    };
\node[left=.1cm of o] (l) {$i =$};
\end{tikzpicture}

==> images/nfa/wtsimpl/term2.tex <==
\begin{tikzpicture}[every node/.style = {shape=rectangle, align=center}]
\node (o) {$strict$} [level distance=0.75cm,sibling distance=1.25cm]
    child { node (o1) {$seq$} [sibling distance=1cm]
      child { node (o11) {$\hlf{l_1}?\hms{m_1}$} }
      child { node (o12) {$\hlf{l_1}!\hms{m_2}$} }
    }
    child { node (o2) {$i$} };
\end{tikzpicture}

==> images/nfa/wtsimpl/term3.tex <==
\begin{tikzpicture}[every node/.style = {shape=rectangle, align=center}]
\node (o) {$strict$} [level distance=0.75cm,sibling distance=1.25cm]
    child { node (o1) {$\hlf{l_1}!\hms{m_2}$} }
    child { node (o2) {$i$} };
\end{tikzpicture}
